Beyond Semantic Understanding: Preserving Collaborative Frequency Components in LLM-based Recommendation

Recommender systems in concert with Large Language Models (LLMs) present promising avenues for generating semantically-informed recommendations. However, LLM-based recommenders exhibit a tendency to overemphasize semantic correlations within users' interaction history. When taking pretrained collaborative ID embeddings as input, LLM-based recommenders progressively weaken the inherent collaborative signals as the embeddings propagate through LLM backbones layer by layer, as opposed to traditional Transformer-based sequential models in which collaborative signals are typically preserved or even enhanced for state-of-the-art performance. To address this limitation, we introduce FreLLM4Rec, an approach designed to balance semantic and collaborative information from a spectral perspective. Item embeddings that incorporate both semantic and collaborative information are first purified using a Global Graph Low-Pass Filter (G-LPF) to preliminarily remove irrelevant high-frequency noise. Temporal Frequency Modulation (TFM) then actively preserves collaborative signal layer by layer. Note that the collaborative preservation capability of TFM is theoretically guaranteed by establishing a connection between the optimal but hard-to-implement local graph fourier filters and the suboptimal yet computationally efficient frequency-domain filters. Extensive experiments on four benchmark datasets demonstrate that FreLLM4Rec successfully mitigates collaborative signal attenuation and achieves competitive performance, with improvements of up to 8.00\% in NDCG@10 over the best baseline. Our findings provide insights into how LLMs process collaborative information and offer a principled approach for improving LLM-based recommendation systems.

==> Tables/dataset_stats.tex <==
\begin{table}[!t]
    \centering
    \caption{Statistics of the preprocessed datasets. Avg. Len denotes the average sequence length of users.}
    \label{tab:dataset_stats}
    \begin{tabular}{@{}lrrrr@{}}
        \toprule
        \textbf{Dataset} & \textbf{\#Users} & \textbf{\#Items} & \textbf{\#Interactions} & \textbf{Avg. Len} \\
        \midrule
        All Beauty & 2,151 & 2,150 & 11,422 & 5.31 \\
        Luxury Beauty & 11,490 & 6,534 & 71,898 & 6.26 \\
        Movies and TV & 309,555 & 86,678 & 1,697,533 & 5.48 \\
        LastFM & 1,090 & 3,646 & 52,551 & 48.21 \\
        \bottomrule
    \end{tabular}
\end{table}
